Arabic Diacritics in the Wild: Exploiting Opportunities for Improved Diacritization

The widespread absence of diacritical marks in Arabic text poses a significant challenge for Arabic natural language processing (NLP). This paper explores instances of naturally occurring diacritics, referred to as "diacritics in the wild," to unveil patterns and latent information across six diverse genres: news articles, novels, children's books, poetry, political documents, and ChatGPT outputs. We present a new annotated dataset that maps real-world partially diacritized words to their maximal full diacritization in context. Additionally, we propose extensions to the analyze-and-disambiguate approach in Arabic NLP to leverage these diacritics, resulting in notable improvements. Our contributions encompass a thorough analysis, valuable datasets, and an extended diacritization algorithm. We release our code and datasets as open source.

==> NOTES-TO-DO.tex <==
DONE����������
Ossama Computational Info
Error analysis: 
Future Work: We will
Appendix C on Ranking
Salman Valid Answer
Order of Appendices
Tanween Alef => Tanwiyn Alif  in text and tables

Bug - ossama/ all in dev.

========

 
Table 1 max diac. discuss  '% Max Diac Words' 

Types of "wildness"

Add mention of {appendix:fulldiacs}

%%%%%%%%%%%%%%%%%%

Wild Diac

DER??

Wild diacs follow up work… clean organize wiki news

Wikinews numbers on exact

Cuts

Appendix

Read all
 

Next steps list and schedule 

Notes

